COLD Decoding: Energy-based Constrained Text Generation with Langevin Dynamics

Many applications of text generation require incorporating different constraints to control the semantics or style of generated text. These constraints can be hard (e.g., ensuring certain keywords are included in the output) and soft (e.g., contextualizing the output with the left- or right-hand context). In this paper, we present Energy-based Constrained Decoding with Langevin Dynamics (COLD), a decoding framework which unifies constrained generation as specifying constraints through an energy function, then performing efficient differentiable reasoning over the constraints through gradient-based sampling. COLD decoding is a flexible framework that can be applied directly to off-the-shelf left-to-right language models without the need for any task-specific fine-tuning, as demonstrated through three challenging text generation applications: lexically-constrained generation, abductive reasoning, and counterfactual reasoning. Our experiments on these constrained generation tasks point to the effectiveness of our approach, both in terms of automatic and human evaluation.

==> abstract-plain.tex <==


Many applications of text generation require incorporating different constraints to control the semantics or style of generated text. These constraints can be hard (e.g., ensuring certain keywords are included in the output) and soft (e.g., contextualizing the output with the left- or right-hand context). In this paper, we present Energy-based Constrained Decoding with Langevin Dynamics (COLD), a decoding framework which unifies constrained generation as specifying constraints through an energy function, then performing efficient differentiable reasoning over the constraints through gradient-based sampling. COLD decoding is a flexible framework that can be applied directly to off-the-shelf left-to-right language models without the need for any task-specific fine-tuning, as demonstrated through three challenging text generation applications: lexically-constrained generation, abductive reasoning, and counterfactual reasoning. Our experiments on these constrained generation tasks point to the effectiveness of our approach, both in terms of automatic and human evaluation.

==> abstract.tex <==
Many applications of text generation require incorporating different constraints to control the semantics or style of generated text. These constraints can be hard (e.g., ensuring certain keywords are included in the output) and soft (e.g., contextualizing the output with the left- or right-hand context). In this paper, we present Energy-based Constrained Decoding with Langevin Dynamics (COLD), a decoding framework which unifies constrained generation as specifying constraints through an energy function, then performing efficient differentiable reasoning over the constraints through gradient-based sampling. COLD decoding is a flexible framework that can be applied directly to off-the-shelf left-to-right language models without the need for any task-specific fine-tuning, as demonstrated through three challenging text generation applications: lexically-constrained generation, abductive reasoning, and counterfactual reasoning. Our experiments on these constrained generation tasks point to the effectiveness of our approach, both in terms of automatic and human evaluation.

==> extras/algorithm_forward.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\KwInput{LM $p_{\theta}$, soft-token history $\ty_{<t}= (\ty_1,\ldots,\ty_{t-1})$.}
\KwOut{Language model probabilities $p_\theta(y_{t}|\ty_{<t})\in \Delta^{\vocab}$.}
%
\textcolor{red}{Todo}
%
\caption{Soft forward pass (left-to-right language model).}
\label{alg:soft-forward}
\end{algorithm}


==> extras/algorithm_postprocess.tex <==
% \begin{algorithm}[t]
% \DontPrintSemicolon
% \KwInput{LM $p_{\text{LM}}$, input canvas $\yb_\text{in}$, update indices $I_{\text{update}}$, number of samples $K$.}
% \KwOut{Sequence $\yb_{1:T}$.}

% %
% \For{$k\in\{1,\ldots,K\}$}{
% %
% $\yb_k=\texttt{soft-decode}(p_{\text{LM}}, \yb_\text{in}, I_{\text{update}})$ \tcp*[r]{decode candidates (Alg.\ref{alg:main})}
% }
% $m_1,\ldots,m_K=\texttt{score}(\yb_1,\ldots,\yb_K)$\\
% return $\yb_k$ with highest score $m_k$
% %
% \caption{Sample-and-rerank.}
% \label{alg:sagga}
% \end{algorithm}


==> extras/tbl_refinement_example_abductive.tex <==
\begin{table}[t]
% \centering
\footnotesize
\begin{tabular}{cc}
%\begin{tabular}{cccccccccccccccccccc}
\toprule
Iteration & {\textbf{Text infilling (abductive reasoning)}} \\
\midrule
Init. template & If it is raining, then there are clouds in the sky. ... Thus, it is not raining. \\
\midrule
1 &  lfadjl eioreo aflsdflj qerlejk aslldfl qleke tqqq\\ 
250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
500 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
750 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1000 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1500 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1750 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2000 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2500 &  There are no clouds in the sky. \\ 
% (target) & Would I ever be able to lead a normal life at Oxford ? \\
\bottomrule
\end{tabular}
\caption{.}
\end{table}

==> extras/tbl_refinement_example_counterfactual.tex <==
\begin{table}[t]
% \centering
\footnotesize
\begin{tabular}{cc}
%\begin{tabular}{cccccccccccccccccccc}
\toprule
Iteration & {\textbf{Semantic similarity (counterfactual reasoning)}} \\
\midrule
Init. context & the medical student \\
Similarity target & joined a prestigious law firm after graduation \\
\midrule
1 &  lfadjl eioreo aflsdflj qerlejk aslldfl qleke tqqq\\ 
250 &  the eioreo cat qerlejk aslldfl qleke tqqq \\ 
500 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
750 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1000 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1500 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1750 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2000 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2500 &  the medical student joined a famous medical practice after graduating \\ 
% (target) & Would I ever be able to lead a normal life at Oxford ? \\
\bottomrule
\end{tabular}
\caption{.}
\end{table}

==> extras/tbl_refinement_example_lexical.tex <==
\begin{table*}[t]
% \centering
\footnotesize
\begin{tabular}{cc}
%\begin{tabular}{cccccccccccccccccccc}
\toprule
Iteration & {\textbf{Lexically-constrained Decoding}} \\
\midrule
Init. constraints & \{\textbf{dog}, \textbf{cat}, \textbf{desk}\} \\
\midrule
1 &  lfadjl eioreo aflsdflj qerlejk aslldfl qleke tqqq\\ 
250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
500 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
750 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1000 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1500 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
1750 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2000 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2250 &  the eioreo \textbf{cat} qerlejk aslldfl qleke tqqq \\ 
2500 &  the \textbf{dog} and \textbf{cat} run under the \textbf{desk} \\ 
% (target) & Would I ever be able to lead a normal life at Oxford ? \\
\bottomrule
\end{tabular}
\caption{.}
\end{table*}

==> tables/ablation.tex <==
\begin{table}[t!]
\footnotesize
    % \setlength{\tabcolsep}{1.0pt}
\begin{minipage}[t]{.5\textwidth}
    \vspace{-3mm}
    \scalebox{.9}{
    \begin{tabular}{lcccc}
        \toprule 
         Models & \makecell{Grammar} & \makecell{Left-\\coher.\\($\xb$-$\yb$)}  & \makecell{Right-\\coher.\\($\yb$-$\zb$)}  & \makecell{Overall-\\coher.\\($\xb$-$\yb$-$\zb$)}  \\ 
         \midrule 
        \modelname (Full) & 4.17 & 3.96 & \bf{2.88} & \bf{2.83} \\
        \modelname  $- f_{\text{sim}}$  & 4.54 & 3.82 & 2.73 & 2.69 \\
        \modelname $- f_{\text{LM}}^{\leftarrow}$ & 4.35 & 3.97 & 2.84 & 2.80 \\
        \modelname $- f_{\text{pred}}$ & \bf{4.61} & \bf{4.07} & 2.75 & 2.77 \\
         \bottomrule
    \end{tabular}}
    \caption{\small Ablation for the effect of different constraints in Eq.(\ref{eqn:energy-abductive}). 
    We do human evaluation on 125 test examples. 
    The best overall coherence is achieved when all the constraints are present.
    }
    \label{tab:ablation_constraints}
    \end{minipage} \hspace{.025\textwidth}
    \begin{minipage}[t]{.45\textwidth}
    \vspace{-3mm}
    \scalebox{.9}{
    \begin{tabular}{rcccc}
        \toprule 
         top-$k$ & \makecell{Grammar} & \makecell{Left-\\coher.\\($\xb$-$\yb$)}  & \makecell{Right-\\coher.\\($\yb$-$\zb$)}  & \makecell{Overall-\\coher.\\($\xb$-$\yb$-$\zb$)}  \\ 
         \midrule 
        2 & \bf{4.38} & \bf{3.99} & 2.88 & 2.92 \\
        5 & 4.27 & 3.71 & 3.04 & 2.87 \\
        10 & 4.09 & 3.84 & \bf{3.09} & \bf{2.94} \\
        50 & 3.95 & 3.62 & 3.07 & 2.87 \\
        100 & 3.80 & 3.54 & 3.03 & 2.84 \\
         \bottomrule
    \end{tabular}}
    \vspace{1mm}
    \caption{\small Ablation for the effect of $k$ in top-$k$ filtering mechanism (\S\ref{ssec:discrete}). We use the same setting as Table~\ref{tab:ablation_constraints}.  
    }
    \label{tab:ablation_topk}
    \vspace{-10pt}
    \end{minipage}
    \vspace{-25pt}
\end{table}
